List-Decodable Subspace Recovery: Dimension Independent Error in Polynomial Time

In list-decodable subspace recovery, the input is a collection of $n$ points $\alpha n$ (for some $\alpha \ll 1/2$) of which are drawn i.i.d. from a distribution $\mathcal{D}$ with a isotropic rank $r$ covariance $\Pi_*$ (the \emph{inliers}) and the rest are arbitrary, potential adversarial outliers. The goal is to recover a $O(1/\alpha)$ size list of candidate covariances that contains a $\hat{\Pi}$ close to $\Pi_*$. Two recent independent works (Raghavendra-Yau, Bakshi-Kothari 2020) gave the first efficient algorithm for this problem. These results, however, obtain an error that grows with the dimension (linearly in [RY] and logarithmically in BK) at the cost of quasi-polynomial running time) and rely on \emph{certifiable anti-concentration} - a relatively strict condition satisfied essentially only by the Gaussian distribution. In this work, we improve on these results on all three fronts: \emph{dimension-independent} error via a faster fixed-polynomial running time under less restrictive distributional assumptions. Specifically, we give a $poly(1/\alpha) d^{O(1)}$ time algorithm that outputs a list containing a $\hat{\Pi}$ satisfying $\|\hat{\Pi} -\Pi_*\|_F \leq O(1/\alpha)$. Our result only needs $\mathcal{D}$ to have \emph{certifiably hypercontractive} degree 2 polynomials. As a result, in addition to Gaussians, our algorithm applies to the uniform distribution on the hypercube and $q$-ary cubes and arbitrary product distributions with subgaussian marginals. Prior work (Raghavendra and Yau, 2020) had identified such distributions as potential hard examples as such distributions do not exhibit strong enough anti-concentration. When $\mathcal{D}$ satisfies certifiable anti-concentration, we obtain a stronger error guarantee of $\|\hat{\Pi}-\Pi_*\|_F \leq \eta$ for any arbitrary $\eta > 0$ in $d^{O(poly(1/\alpha) + \log (1/\eta))}$ time.

==> content/lower-error-old.tex <==
%!TEX root = ../main.tex


\section{List-Decodable Subspace Recovery with Arbitrarily Tiny Error}
% Recall the subspace recovery problem. Here, $\alpha n$ fraction of the points lie in $k$-dimensional subspace and are distributed as $\mathcal{N}(0,\Sig)$. The projection on to this subspace is given by a $n\times n$, rank-$k$ matrix $\Sigma_*$.  Let $w$ be an indicator vector. We recall the following set of constraints in variables $w$ and $\Sig$

In this section, we describe an efficient algorithm for list-decodable subspace recovery with arbitrarily small error at the cost of returning a polynomial (in the dimension $d$) size list.



\begin{theorem}[Large-List Subspace Recovery, Theorem \ref{thm:large_list_sr} restated]\label{thm:large-list-rounding}
Let $\sub_{\cD}(\alpha, \Sigma_*)$ be such that $\Sigma_*$ has rank $r$ and condition number $\kappa$, and  $\cD$ is $k$-certifiably $(c,\alpha/2)$-anti-concentrated. For any $\eta >0$, there exists an algorithm that takes input $n \geq n_0 = (kd\log(d))^{O(k)}$ samples from $\sub_{\cD}(\alpha, \Sigma_*)$ and outputs a list $\cL$ of size $O(1/\alpha^{k\log(r\kappa/\eta)})$ of projection matrices such that with probability at least $0.99$ over the draw of the sample and the randomness of the algorithm, there is a $\hat{\Pi} \in \cL$ satisfying $\|\hat{\Pi} - \Pi_*\|^2_F \leq \eta$. The algorithm has time complexity at most $n^{O(k^2\log(r\kappa/\eta))}$. 
\end{theorem}


Let $\cA_{w,\Pi}$ be the following system of polynomial inequality constraints in indeterminates $w,\Pi$.
\begin{equation}
  \cA_{w,\Pi}\colon
  \left \{
    \begin{aligned}
      &&
      \textstyle\sum_{i\in[n]} w_i
      &= \alpha n\\
      &\forall i\in [n].
      & w_i (\II - \Pi) x_i
      & = 0 \\
      &\forall i\in [n].
      & w_i^2
      & = w_i \\
      &
      & \Pi^2
      & = \Pi\\
      &
      &\Tr(\Pi)
      &= r\\
      &\forall Q 
      &\frac{1}{\alpha n} \sum_{i \leq n} w_i \Paren{x_i^{\top} Q x_i}^{2t} 
      &\leq (Ct)^t \Paren{\frac{1}{\alpha n} \sum_{i \leq n} w_i \Paren{x_i^{\top} Q x_i}^2}^t
    \end{aligned}
  \right \}
\end{equation}
% \begin{equation}
%   \cA_{w,\Pi}\colon
%   \left \{
%     \begin{aligned}
%       &&
%       \textstyle\sum_{i\in[n]} w_i
%       &= \alpha n\\
%       &\forall i\in [n].
%       & w_i (\II - \Pi) x_i
%       & = 0 \\
%       &\forall i\in [n].
%       & w_i^2
%       & = w_i \\
%       &
%       & \Pi^2
%       & = \Pi\\
%       %&
%       %&\Pi
%       %& = VV^{\top}\\
%       &
%       &\Tr(\Pi)
%       & = r\\
%     \end{aligned}
%   \right \}
% \end{equation}
%\Pnote{all commentary should happen  only in intro/overview. COmmenting out the prose here. why do we have the $\Pi = VV^T$ constraint?}
%Our algorithm searches over high-entropy pseudo-distributions over $w$ and $\Sig$ such that the aforementioned constraints are satisfied. \FIXME{reasons for searching over high-entropy distributions.} Intuitively, the key fact we use is that a degree-$t$ pseudo-distribution behaves quite like a real distribution when we compute pseudo-expectations w.r.t. degree-$t$ polynomials.
%\FIXME{You shouldn't need moment matching constraints. Should do all proofs with just the constraint above.}


Our algorithm finds a pseudo-distribution consistent  with $\cA_{w,\Pi}$. It then uses the large-list rounding algorithm as a first step to get a polynomial (in $d$) size list that contains a subspace that is $\eta$-close in Frobenius norm to the range space of $\Sigma_*$. Finally, we apply a pruning procedure to obtain a $O(1/\alpha)$ size from the large list procedure.





%\begin{mdframed}[nobreak=true]
%  \begin{algorithm} Large-List Subspace Recovery via Rounding
%    \label[algorithm]{alg:rounding_large_list}\mbox{}
%    \begin{description}
%    \item[Given:]
%    Sample $\cS = \{x_1, x_2, \ldots x_n \} = \cI \cup \cO$ of size $n$ drawn according to $\sub_{D}(\alpha,\Sigma_*)$ such that the $\cD$ is $k$-certifiably $(c,\delta)$-anti-concentrated, has mean $0$ and the condition number of $\Sigma_*$ is $\kappa$. Accuracy parameter $\eta > 0$.
%      \item[Operation:] \textrm{ } \\
%      \vspace{-0.3in}
%      \begin{enumerate}
%        \item Let $t  = \Delta \cdot k \log(r\kappa/\eta)$ for a fixed constant $\Delta$. Compute a pseudo-distribution $\tmu$ of degree $t+2k$ satisfying $\cA_{w,\Pi}$ and minimizing $\Norm{\sum_{i\leq n} \pE w_i}_2^2$.
%        \item Repeat $\ell= O(1/\alpha^t)$ times:
%      \begin{enumerate}
%      \item Let $S \subset [n]$ such that $|S| = \alpha n$. Draw $S$ with probability proportional to ${n \choose S} \pE_{\tmu}[w_S]$.
%      \item Let $\tilde{\Pi} = \frac{\pE_{\tmu}[ w_s \Pi]}{\pE_{\tmu}[w_S]}$ be the corresponding matrix. Compute the Eigenvalue Decomposition of $\tilde{\Pi} = \tilde{U}\tilde{\Lambda}\tilde{U}^{\top}$ and let $\hat{\Pi} = \tilde{U}_{r}\tilde{U}^{\top}_{r}$, where $\tilde{U}_{r}$ are the eigenvectors corresponding to the top-$r$ eigenvalues of $\tilde{\Pi}$.
%      \item Add $\hat{\Pi}$ to the list $\cL'$.
%    \end{enumerate}
%  \end{enumerate}
%    \item[Output:]
%      A list $\cL' \subseteq \R^d$ of size $O(1/\alpha^t)$ containing a Projection matrix $\hat{\Pi} \in \cL'$ satisfying $\|\hat{\Pi} -\Pi_*\|^2_F < \eta$.
%    \end{description}
%  \end{algorithm}
%\end{mdframed}


\begin{mdframed}[nobreak=true]
  \begin{algorithm} List-Decodable Subspace Recovery
    \label[algorithm]{alg:subspace-recovery}\mbox{}
    \begin{description}
    \item[Given:]
    Sample $\cS = \{x_1, x_2, \ldots x_n \} = \cI \cup \cO$ of size $n$ drawn according to $\sub_{D}(\alpha,\Sigma_*)$ such that the $\cD$ is $k$-certifiably $(c,\delta)$-anti-concentrated, has mean $0$ and the condition number of $\Sigma_*$ is $\kappa$.
    %Accuracy parameter $\eta > 0$. %, $t = O(\log r)$.
      \item[Operation:] \textrm{ }\\
      \vspace{-0.3in}
      \begin{enumerate}
        \item Find a degree $O(1/\alpha^4 \eta^4)$ pseudo-distribution $\tilde{\mu}$ satisfying $\cA_{w,\Pi}$ that minimizes $\|\pE[w]\|_2$.
        \item For each $i \in [n]$ such that $\pE_{\tmu}[w_i] > 0$, let $\hat{\Pi}_i = \frac{\pE_{\tmu}[w_i \Pi]}{\pE_{\tmu}[w_i]}$. Otherwise, set $\hat{\Pi}_i =0$.
        \item Take $J$ be a random multi-set formed by union of $O(1/\alpha)$ independent draws of $i \in [n]$ with probability $\frac{\pE[w_i]}{\alpha n}$.
        \item Output $\cL = \{\hat{\Pi}_i \mid i \in J\}$ where $J \subseteq [n]$.
      \end{enumerate}
    \item[Output:] A list $\cL$ of size $O(1/\alpha)$ containing $\hat{\Pi}$ such that $\Norm{\hat{\Pi}-\Pi_*}_F \leq \eta$.   
     \end{description}
  \end{algorithm}%\label{alg:main}
\end{mdframed}




% \begin{mdframed}[nobreak=true]
%   \begin{algorithm} Large List Rounding
%     \label[algorithm]{alg:rounding_large_list}\mbox{}
%     \begin{description}
%     \item[Given:] 
%     A pseudo-distribution $\tmu$ of degree $t+2k$ satisfying $\cA_{w,\Pi}$ and minimizing $\Norm{\sum_{i\leq n} \pE w_i}_2^2$ such that $t =  \Delta \cdot \left(\frac{\log^5(1/\alpha)\log(r\kappa/\eta)}{\alpha^2}\right)$, for a large constant $\Delta$, accuracy parameter $\eta >0$. 
%       \item[Operation:] Repeat $\ell= O(1/\alpha^t)$ times:
%       \begin{enumerate}
%       \item Let $S \subset [n]$ such that $|S| = \alpha n$. Draw $S$ with probability proportional to ${n \choose S} \pE_{\tmu}[w_S]$.
%       \item Let $\tilde{\Pi} = \frac{\pE_{\tmu}[ w_s \Pi]}{\pE_{\tmu}[w_S]}$ be the corresponding matrix. Compute the Eigenvalue Decomposition of $\tilde{\Pi} = \tilde{U}\tilde{\Lambda}\tilde{U}^{\top}$ and let $\hat{\Pi} = \tilde{U}_{r}\tilde{U}^{\top}_{r}$, where $\tilde{U}_{r}$ are the eigenvectors corresponding to the top-$r$ eigenvalues of $\tilde{\Pi}$.
%       \item Add $\hat{\Pi}$ to the list $\cL'$.
%     \end{enumerate}
%     \item[Output:]
%       A list $\cL' \subseteq \R^d$ of size $O(1/\alpha^t)$ containing a Projection matrix $\hat{\Pi} \in \cL'$ satisfying $\|\hat{\Pi} -\Pi_*\|^2_F < \eta$.
%     \end{description}
%   \end{algorithm}
% \end{mdframed}


\subsection{Analysis of Algorithm \ref{alg:subspace-recovery}.}

Our proof of Theorem \ref{thm:large-list-rounding} is based on the following four pieces. 
The key technical piece is the following consequence of the constraint system $\cA_{w,\Pi}$ in the low-degree SoS proof system.

\begin{lemma} \label{lem:main-sosized-fact}
Given $\delta >0 $ and any $t \in \N$, and an instance of $\sub_{\cD}(\alpha, \Sigma_*)$, such that the inlier distribution $\cD$ has mean $0$ and is $k$-certifiably $(C,\delta)$-anti-concentrated,
\[
\cA_{w,\Pi} \sststile{2k+t}{\Pi,w} \Set{ w(\cI)^t \Norm{\Pi-\Pi_*}_F^k = w(\cI)^t 2^{k/2} \Tr(M\Pi_*M)^{k/2} \leq (2r\kappa)^{k/2}\delta^t}\mper
\]
where $\kappa$ is the condition number of $\Sigma_*$ and $\Pi_*$ is the corresponding rank-$r$ Projection matrix.
%Write the first fact in the onenote doc without pseudo-expectations.
\end{lemma}

Similar to the previous section, we rely on the following consequence of high-entropy constraints on the the pseudo-distribution $\tmu$.
\begin{fact}[Large weight on inliers from high-etropy constraints] \label{fact:high-entropy-pseudo-distributions-2}
Let $\tmu$ pseudo-distribution of degree $\geq t$ that satisfies $\cA_{w,\Pi}$ and minimizes $\Norm{\pE_{\tmu'} \sum_{i \in [n]} w_i}_2$. Then, $\frac{1}{|\cI|^t} \pE \left[\Paren{\sum_{i \in \cI}  w_i }^t\right] \geq \alpha^t$.
\end{fact}

The above two lemmas allow us to complete the proof of correctness of Algorithm \ref{alg:rounding_large_list}.




% Theorem \ref{thm:algorithm-analysis} follows easily by combining the above claims :
% \begin{proof}[Proof of Theorem ~\ref{thm:algorithm-analysis}]

% %It follows from Theorem \ref{thm:cert_anti_conc_gaussians} that $\cN(0,\Sigma_*)$ is $O(\log^5(1/\delta)/\delta^2)$-certifiably $(c,\delta)$-anti-concentrated. 
% Recall, $\cD$ is $k$-certifiably $(c,\alpha/2)$-anti-concentrated, and thus it follows from Lemma \ref{lem:certifiable_anti_conc_sampling} that the uniform distribution on $\cI$ is also $O(k)$-certifiably $(c,\alpha)$-anti-concentrated if the number of samples are at least $n_0 =  (d\log(d)/\alpha^2)^{\widetilde{O}(k)}$. 

% We begin by observing that the system of constraints $\cA_{w,\Pi}$ is feasible when we set $w_i$ to indicate the inliers, and $\Pi =\Pi_*$. 
% Next, the hypothesis of Lemma \ref{lem:large-list-rounding} is now satisfies for $\eta = 0.1$, Algorithm \ref{alg:rounding_large_list} runs in time $n^{\widetilde{O}(\log(r\kappa)k)}$ and outputs a list $\cL'$ of size $(1/\alpha)^{\widetilde{O}(\log(r\kappa)k)}$ such that with probability at least $99/100$, it contains a projector $\tilde{\Pi}$ satisfying $\|\tilde{\Pi} - \Pi_*\|^2_F \leq 0.1$. Recall, $\Pi_*$ is the projector corresponding to $\Sigma_*$ and let $\zeta_1$ be the event that $\cL'$ contains $\Pi_*$. 

% Conditioning on $\zeta_1$,  we now have a list satifying the hypothesis for Lemma \ref{lem:pruning-algorithm} and access to $O(1/\alpha)$ fresh samples ($\gamma = 1$) we can conlcude that with probability $99/100$ Algorithm \ref{alg:pruning} outputs a list of size $O(1/\alpha)$ which containts a projection matrix $\hat{\Pi}$ satisfying $\|\hat{\Pi}-\Pi_*\|^2_F \leq \widetilde{O}(\kappa^4 \log(r)/\alpha^2)$, as desired. Let $\zeta_2$ be the event that Algorithm \ref{alg:pruning} succeeds. Therefore, union bounding over $\zeta_1$ and $\zeta_2$ implies Algorithm \ref{alg:subspace-recovery}  succeeds with probability at least $9/10$. 
% The overall running time is dominated by Algorithm \ref{alg:rounding_large_list}, which completes the proof. 


%Therefore, the correctness of Theorem \ref{thm:algorithm-analysis} follows simply from Lemma \ref{lem:pruning-algorithm} since with probability $99/100$, $\cL$ contains a Projection matrix $\hat{\Pi}$ such that $\|\hat{\Pi} - \Pi_*\|^2_F \leq \tau$. Further, since Algorithm \ref{alg:pruning} iterates only $O(1/\alpha)$ times, and in each iteration adds at most one projection matrix to $\cL$, $|\cL| \leq O(1/\alpha)$.

%Since we require the uniform distribution on the inliers to be $k$-certifiably $(C,\delta)$-anti-concentrated, it follows from Lemma \ref{lem:certifiable_anti_conc_sampling} that  samples suffice.
%Next, we analyze the running time of Algorithn \ref{alg:subspace-recovery}. The running time is dominated by Step 2, where we find a degree $(2t + k)$ pseudo-distribution $\tmu$ that minimizes  $\Norm{\sum_{i = 1}^n\pE[w_i]}^2_2$. Since $w$ is an $n$-dimensional vector and $\Pi$ is a $d \times d$ matrix, it follows from Fact \ref{fact:efficient_sos_opt} that we can compute $\tmu$ in $(n+d^2)^{2t+k} = (kd)^{O(tk + k^2)}$ time.  Algorithms \ref{alg:rounding_large_list} and \ref{alg:pruning} run in $\textrm{poly}(n,d, 1/\alpha^t)$ time and thus the total running time is bounded by $(kd)^{O(tk + k^2)}$.
% \end{proof}





\subsection{Analyzing $\cA_{w,\Pi}$: Proof of Lemma ~\ref{lem:main-sosized-fact}}


% \begin{fact}[Indicator Polynomial]
% For any $\delta >0$, there exists a even univariate polynomial $p(x)$ of degree $m = \widetilde{\Omega}(1/\delta^2)$ such that
% \begin{enumerate}
%   \item p(0)=1.
%   \item if $x \leq \delta$, $p(x) = 1\pm\delta $.
%   %If $\iprod{x, v}^2 \leq \delta^2 \expecf{}{\iprod{x,v}^2}$, then $|p(\iprod{x,v})-1| \leq \delta$
%   \item $\expecf{x\sim \cN(0,1)}{p^2(x)} \leq 2\delta$
%   %$\expecf{}{p^2(\iprod{x,v})} \leq 2\delta$
% \end{enumerate}
% \end{fact}
%\FIXME{polynomials etc should appear in the proof since they come from the definition of certifiable anti-concentration.}

We first show that covariance of  all large enough subsamples of certifiably anti-concentrated samples have lower-bounded eigenvalues. Recall, for a PSD matrix $\Sigma_*$,  $U \Lambda U^{\top}$ denotes the Eigenvalue Decomposition and $\Pi_* = UU^{\top}$ denotes the corresponding rank-$r$ Projection matrix.


% \begin{lemma}[Spectral Lower Bound on Subsamples via AntiConcentration]
% Let $\cS = \{x_1, x_2, \ldots x_n\} \subseteq \R^d$ be $k$-certifiably $(C,\delta)$-anti-concentrated with covariance $\Sigma_*$. Then,
% %Anti-concentration...using polynomial..
% \begin{equation}
%  \Set{w_i^2 = w_i \forall i}  \sststile{k}{w} \Set{\frac{1}{n} \sum_{i=1}^n w_i \iprod{x_i,v}^2 \geq \left( \frac{1}{n} \sum_{i =1}^n w_i- 4\delta \right) \delta^2 v^{\top} \Sigma_* v} \mper

\begin{lemma}[Covariance of Subsets of Certifiably Anti-Concentrated Distributions]
\label{lem:subset_cov_anti_conc}
%Let $\cS = \{x_1, x_2, \ldots x_n\} \subseteq \R^d$ be $k$-certifiably $(C,\delta)$-anti-concentrated with $\frac{1}{n} \sum_{x \in \cS} xx^{\top} = \Sigma$.
For any $v \in \R^d$ such that $\Pi_*v = v$ and $\Norm{v}_2^2 =1$, 
%Anti-concentration...using polynomial..
\begin{equation}
\Set{w_i^2 = w_i \mid \forall i} \sststile{2k}{w,v} \Set{\frac{1}{\alpha n} \sum_{i \in \cI} w_i\iprod{x_i, v}^2 \geq  \delta^2 \Paren{\frac{1}{n} \sum_{i \in \cI} w_i-C\delta} \norm{\Pi_* v}_2^{2}}\mcom
\end{equation}

\end{lemma}

\begin{proof}
Let $p$ be the degree $k$ polynomial provided by Definition~\ref{def:certifiable-anti-concentration-homogenous} applied to $\cI$. Thus, for each $1 \leq i \leq n$, and any $v \in \R^d$ such that $\norm{v}_2 \leq 1$, we must have:
\[
\sststile{2k}{\Pi,w} \Set{\iprod{x_i,v}^2 + \delta^2 \norm{v}_2^2 p^2\paren{\iprod{ x_i,v}} \geq \delta^2 }\mper
\]
Observe that
\[
\Set{w_i^2 = w_i} \sststile{2}{w_i} \Set{w_i \geq 0}\mper
\]

% and,
% \[
% \Set{w_i^2 = w_i} \sststile{2j}{w_i} \Set{\iprod{\Sigma^{\dagger/2} x_i,v}^j}\mcom
% \]

Using the above along with \eqref{eq:sos-addition-multiplication-rule} for manipulating SoS proofs, we must have:
\[
\Set{w_i^2 = w_i \mid \forall i} \sststile{2k}{w} \Set{\frac{1}{\alpha n} \sum_{i \in \cI} w_i \iprod{x_i,v}^2 + \delta^2 \frac{1}{\alpha n} \sum_{i \in \cI} w_i \norm{v}_2^2 p^2\paren{\iprod{x_i,v}} \geq \delta^2 \frac{1}{\alpha n} \sum_{i \in \cI} w_i \norm{v}_2^2}\mper
\]
Rearranging yields:
\begin{equation}
\Set{w_i^2 = w_i \mid \forall i} \sststile{2k}{w} \Set{\frac{1}{\alpha n} \sum_{i \in \cI} w_i\iprod{x_i,v}^2 \geq  \delta^2 \frac{1}{\alpha n} \sum_{i \in \cI} \norm{v}_2^{2}-\delta^2 \frac{1}{\alpha n} \sum_{i \in \cI} w_i \norm{v}_2^2 p^2\paren{\iprod{x_i,v}} }\mper \label{eq:eq-poly-1}
\end{equation}

Next, observe that $\Set{w_i^2 = w_i} \sststile{2}{w_i} \Set{(1-w_i)= (1-w_i)^2 \geq 0}$. Thus, $\Set{w_i^2 = w_i} \sststile{2}{w_i} \Set{w_i \leq 1}$. As a consequence, $\Set{w_i^2 = w_i} \sststile{k+2}{w_i} \Set{w_i p^2(\iprod{x_i , v })\leq p^2(\iprod{x_i , v })}$. Summing up over $1 \leq i \leq n$ yields:

\[
\Set{w_i^2 = w_i \mid \forall i} \sststile{2k}{w} \Set{\frac{1}{\alpha n} \sum_{i \in \cI} w_i \norm{v}_2^2 p^2\paren{\iprod{x_i,v}}\leq \frac{1}{\alpha n} \sum_{i \in \cI} \norm{v}_2^2 p^2\paren{\iprod{x_i,v}} \leq C\delta } \mcom 
\]
where in the final inequality on the RHS above, we used the second condition from Definition~\ref{def:certifiable-anti-concentration-homogenous} satisfied by $\cS$.
Plugging this back in \eqref{eq:eq-poly-1}, we thus have:

\begin{equation}
\Set{w_i^2 = w_i \mid \forall i} \sststile{2k}{w,\Pi} \Set{\frac{1}{n} \sum_{i = 1}^n w_i\iprod{x_i,v}^2 \geq  \delta^2 \Paren{\frac{1}{n} \sum_{i = 1}^n w_i-C\delta} }\mcom
\end{equation}
as desired.


% \begin{equation}
% \label{eqn:poly_id}
%     %\left\{ (p(\iprod{x_i, v}) -1)^2 \leq \delta \mid \langle x_i,v\rangle^2 \leq \delta^2 \E \langle x_i ,v\rangle^2 \right\}
%     \sststile{k}{v} \left\{ \iprod{x_i, v}^2 + \delta^2 \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] p^2(\iprod{x_i, v}) \geq \frac{\delta^2}{2} \E_{x_i \sim \cS}\left[\iprod{x_i, v}^2\right] \right\}
% \end{equation}
% %$z^2 + \delta^2 v^{\top}\Sig_2 v\cdot p^2\left(w_i\iprod{x_i, v}\right) \geq (\delta^2 -\delta^3)v^{\top} \Sig v$.
% %\FIXME{convert this into SOS notation. }
% To prove the aformentioned inequality, we first consider the case when $\langle x_i,v\rangle^2 \leq \delta^2 \E_{x_i \sim \cS}\left[\iprod{x_i, v}^2\right]$.
% \begin{equation*}
% \begin{split}
% \left\{  \langle x_i,v\rangle^2 \leq \delta^2 \E_{x_i \sim \cS}\left[\iprod{x_i, v}^2\right] \right\} & \sststile{k}{v} \left\{ \iprod{x_i, v}^2 + \delta^2 \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] p^2(\iprod{x_i, v}) \geq  \delta^2 \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] p^2(\delta^2 \E \iprod{x_i,v}^2 )  \right\} \\
% &  \sststile{k}{v} \left\{ \iprod{x_i, v}^2 + \delta^2 \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] p^2(\iprod{x_i, v}) \geq \delta^2 \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] /2 \right\}
% \end{split}
% \end{equation*}
% Next, we consider the case when $\langle x_i,v\rangle^2 > \delta^2 \E_{x_i \sim \cS}\left[\iprod{x_i, v}^2\right]$. Recall, using certifiable anti-concentration, we can now derive via a degree $k$ sos proof that $p(\iprod{x_i, v})^2\geq (1-\delta^2)$. Therefore,
% \begin{equation*}
% \begin{split}
% \{  \langle x_i,v\rangle^2 \geq \delta^2 \E \langle x_i ,v\rangle^2, \} & \sststile{k}{v} \left\{ \iprod{x_i, v}^2 + \delta^2\E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] p^2(\iprod{x_i, v}) \geq  \delta^2 (1-\delta^2) \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right]  \right\} \\
% &  \sststile{k}{v} \left\{\iprod{x_i, v}^2 + \delta^2c p^2(\iprod{x_i, v}) \geq \frac{ \delta^2 \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right]}{2}  \right\}
% \end{split}
% \end{equation*}
% Thus, scaling both sides of Equation \ref{eqn:poly_id} with $w_i$ and averaging over all $i \in [n]$, we have
% \begin{equation*}
% \{ w_i= w_i^2,  \forall i \} \sststile{k}{v,w} \left\{ \frac{1}{n} \sum_{i \in [n]} \Paren{w_i\iprod{x_i,v}^2+ \delta^2 w_i \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] \cdot p^2\left(\iprod{x_i, v} \right)} \geq  \frac{ \delta^2  \sum_{i\in [n]}w_i }{2n}\E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] \right\}
% \end{equation*}
% Rearranging, we obtain that
% \begin{equation}
% \label{eqn:anti_proof}
% \begin{split}
%     \{ w_i= w_i^2,  \forall i \} & \sststile{k}{v,w} \left\{ \frac{1}{n} \sum_{i \in [n] } w_i\iprod{x_i, v}^2  \geq \frac{1}{2} \delta^2  \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] \left( \frac{\sum_{i\in[n]}w_i}{n} -  \frac{1}{n} \sum_{i \in [n]} w_i p^2(\iprod{x_i, v} ) \right) \right\}  \\
%     \{ w_i= w_i^2,  \forall i \} & \sststile{k}{v,w} \left\{\frac{1}{n} \sum_{i \in [n] } w_i\iprod{x_i, v}^2 \geq \frac{1}{2} \delta^2  \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] \Paren{\frac{\sum_{i\in[n]}w_i}{n}-  \frac{1}{n} \sum_{i \in [n]}  p^2\left(\iprod{x_i, v} \right)} \right\}
%     %\left\{  \right\}
%     %& \geq \frac{1}{2} \delta^2  \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] \Paren{\frac{\sum_{i\in[n]}w_i}{n}-  \frac{1}{n} \sum_{i \in [n]}  p^2\left(\iprod{x_i, v} \right)}
% \end{split}
% \end{equation}
% where the last inequality follows from non-negativity of $p^2$.
% Note, when $\E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] =0$, the inequality trivially holds. Therefore, we focus on the case where $\E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] > 0$. Recalling that $k$-certifiable $(2, 2 \delta)$-anti concentration of $\cS$ implies that $p^2$ is small on average, we have
% \begin{equation}
% \label{eqn:polynomial_expectation}
% \begin{split}
%     \left\{ \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right] > 0 \right\} \sststile{k}{v} \left\{\E_{x_i \sim \cS} \iprod{x_i, v}^2 \frac{1}{n}\sum_{i \in [n]} p^2(\iprod{x_i v}) \leq 4 \delta \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right]
%     \right\}
% \end{split}
% \end{equation}
% Combining equations \ref{eqn:polynomial_expectation} and \ref{eqn:anti_proof}, we can conclude

% \begin{equation}
% %\label{eqn:certificate_near_gaussian}
% \Set{w_i^2 = w_i \forall i}  \sststile{k}{w,v} \Set{\frac{1}{n} \sum_{i=1}^n w_i \iprod{x_i,v}^2 \geq \left( \frac{\sum_{i =1}^n w_i}{n} - 4\delta \right) \delta^2  \E_{x_i \sim \cS} \left[\iprod{x_i, v}^2\right]}
% \end{equation}

\end{proof}

% \begin{lemma}
% \begin{equation}
% \sststile{2t}{\Sig} \Set{\trace{\Sig - \Sigma_*}^{2t} \leq d - \trace{\Sig \Sigma_*}}\mper
% \end{equation}
% %Relating trace powers of projectors to frobenius error.
% \end{lemma}


\begin{lemma}[Technical SoS fact about Powering]
\label{lem:powering}
For indeterminates $a,b,Z$ and any $t \in \N$,
\begin{equation}
 \{a \geq 0, b \geq 0, (a-b)Z  \leq 0 \} \sststile{t}{a,b} \left\{ (a^{t} - b^{t})Z \leq 0 \right\}
\end{equation}

\end{lemma}


\begin{proof}
We have:
\[
\Set{a \geq 0, b \geq 0} \sststile{t}{a} \Set{\sum_{i = 0}^{t-1} a^{t-1-i}b^{i} \geq 0}\mper
\]
Using the  above identity with \eqref{eq:sos-addition-multiplication-rule} yields:
\[
\Set{a \geq 0, b \geq 0, (a-b)Z \leq 0 } \sststile{t}{a,b} \left\{ \Paren{a-b}\Paren{\sum_{i = 0}^{t-1} a^{t-1-i}b^{i}} Z \leq 0 \right\}\mper
\]
Using the identity: $\Paren{a^2-\delta}\Paren{\sum_{i = 0}^{t-1} a^{t-1-i}b^{i}} = a^{t}-b^t$, we finally obtain:
\[
\Set{a \geq 0, b \geq 0, (a-b)Z \leq 0 } \sststile{t}{a,b} \left\{ \Paren{a^{t}-b^t} Z\leq 0\right\}\mper
\]

\end{proof}


%\end{lemma}\FIXME{add proof for this lemma in appendix.}
\begin{proof}[Proof of Lemma \ref{lem:main-sosized-fact}]
 % and the empirical covariance $\expecf{x_i \sim \cI}{x_i x_i^{\top}} = \Sig_*$.
Let $v$ be a unit vector such that $\Pi_* v = v$. 
From Lemma \ref{lem:subset_cov_anti_conc} we have: % to the set $\cI$. Observe, the uniform distribution on $\cI$ is $k$-certifiably $(C,\delta)$-anti-concentrated. Thus,

\begin{equation}
    \Set{w_i^2 = w_i \text{ }\mid \forall i}  \sststile{2k}{w} \Set{\frac{1}{|\cI|} \sum_{i\in \cI} w_i \iprod{x_i,v}^2  \geq \delta^2\left( w(\cI) - C\delta \right)  }
\end{equation}

Let $M = \II-\Pi$. Since $x_i = \Pi_* x_i$, we have the following polynomial identity  (in indeterminates $\Pi,v$) for any $i$:

\[
\iprod{ \Pi_* x_i, \Pi_* M  v} = \iprod{M x_i, v}\mper
\]

By using the \eqref{eq:sos-substitution} for manipulating SoS proofs and substituting $v$ with the polynomial $\Pi_* M  v$, we thus obtain:

\begin{equation}
    \Set{\forall i \in [n] \textrm{  } w_i^2 = w_i }  \sststile{2k}{w,v} \Set{\frac{1}{|\cI|} \sum_{i\in \cI} w_i \iprod{M x_i,v}^2 \Norm{\Pi_* M  v}_2^{k-2} \geq \delta^2\left( \frac{\sum_{i \in \cI} w_i}{|\cI|} - C\delta \right) \Norm{\Pi_* M  v}_2^{k}} \label{eq:pre-0-expression}
\end{equation}






Next, observe that $\cA_{w,\Pi} \sststile{2}{w,\Pi} \Set{ w_i M x_i = 0 \text{ } \forall i}$ and thus,
\[
\cA_{w,\Pi} \sststile{4}{w,v,\Pi} \Set{ \iprod{w_i M x_i,v}^2 = w_i\iprod{M x_i,v}^2 =  0 \text{ } \forall i}\mper
\]
Combining this with \eqref{eq:pre-0-expression}, we thus have:
\begin{equation}
    \cA_{w,\Pi}  \sststile{2k}{w,v} \Set{0 \geq \delta^2\left(w(\cI)  - C\delta \right) \Norm{\Pi_* M v}_2^{k}} \label{eq:post-0-expression}
\end{equation}

Using \eqref{eq:sos-addition-multiplication-rule} to multiply throughout by the constant $1/\delta^2$ yields:

\begin{equation}
     \cA_{w,\Pi} \sststile{2k}{w,v} \Set{0 \geq \left(w(\cI)  - C\delta \right) \Norm{\Pi_* M  v}_2^{k}} \label{eq:post-0-expression_2}
\end{equation}



Let $g \sim \cN(0,I)$. Then, using the above with the substitution $v = g$, and certifiable hypercontractivity of Gaussians (Fact~\ref{fact:certifiable_hypercontractivity_gaussians}), we have:
\begin{multline}
\label{eq:bound_useful}
\cA_{w,\Pi} \sststile{2k}{v,w} \Biggl\{ w(\cI) k^{-k} \E (g^{\top} M\Pi_*M g)^{k/2} \leq  \E (g^{\top} M\Pi_*M g)^{k/2} w(\cI) \E \Norm{\Pi_* M g}_2^k\\ = w(\cI) (\E g^{\top} M\Pi_*M g)^{k/2} = w(\cI) \Tr(M\Pi_*M)^{k/2} \leq w(\cI)\E (g^{\top} M\Pi_*M g)^{k/2} \Biggr\}\mcom
\end{multline}
where the inequality follows from the SoS Hölder's inequality.

Thus, we have:

\begin{equation}
    \cA_{w,\Pi}  \sststile{2k}{w,v} \Set{w(\cI) \Tr(M\Pi_*M)^{k/2} \leq k^k C\delta \Tr(M\Pi_*M)^{k/2} } \label{eq:post-0-expression-2}
\end{equation}



Next,
\[
\Set{\Pi^2 = \Pi} \sststile{2}{\Pi} \Set{\Norm{\Pi}_F^2 = \Tr(\Pi^2) = \Tr(\Pi)=r}\mper
\]
And also,
\[
\Set{\Pi^2 = \Pi} \sststile{2}{\Pi} \Set{M^2 = (I-\Pi)^2 = I -2\Pi + \Pi^2 = I-\Pi = M}\mper
\]
Thus,
% \begin{equation*}
% \begin{split}
% \cA_{w,\Pi} \sststile{2}{\Pi} \Biggl\{ \Norm{\Pi-\Pi_*}_F^2 &= \Norm{\Pi}_F^2 + \Norm{\Pi_*}_F^2 - 2 \Tr(\Pi \Pi_*) = 2r - 2 \Tr(\Pi \Pi_*) \\
% &= 2 \Tr((I-\Pi)\Pi_*) = 2\Tr(M\Pi_*) = 2 \Tr(M^2\Pi_*) = 2\Tr(M\Pi_*M)\Biggr\}\mper
% \end{split}
% \end{equation*}
\begin{equation*}
\begin{split}
\cA_{w,\Pi} \sststile{2}{\Pi} \Biggl\{ \Norm{\Pi-\Pi_*}_F^2 & = \Norm{\Pi}_F^2 + \Norm{\Pi_*}_F^2 - 2 \Tr(\Pi \Pi_*) = 2r - 2 \Tr(\Pi \Pi_*) \\
& = 2 \Tr((I-\Pi)\Pi_*) = 2\Tr(M\Pi_*) = 2 \Tr(M^2\Pi_*) = 2\Tr(M\Pi_*M)\Biggr\}\mper
\end{split}
\end{equation*}

Thus, we have:


\begin{equation}
    \cA_{w,\Pi}  \sststile{2k}{w,v} \Set{w(\cI) \Norm{\Pi-\Pi_*}_F^{k} \leq k^k C\delta \Norm{\Pi-\Pi_*}_F^k } \label{eq:post-0-expression-3}
\end{equation}




Applying Lemma~\ref{lem:powering} with $a = \frac{1}{|\cI|} \sum_{i \in\cI} w_i$, $b = C\delta$ and $Z = \Norm{\Pi_* M  v}_2^{k}$, we obtain:
\begin{equation}
     \cA_{w,\Pi} \sststile{2k + t}{w,v} \Set{0 \geq  \Paren{w(\cI)^t - \paren{C\delta}^t} \Norm{\Pi_* M  v}_2^{k}} \label{eq:post-0-expression_3}
\end{equation}
% %\FIXME{A:I think the degree here should be 2k + t using the derivation rules.}
% Let $\lambda_{max}$ be the largest eigenvalue of  $\Sigma_*$. By applying \eqref{eq:sos-addition-multiplication-rule} and multiplying by $1/\lambda_{max}$ throughout, we can work with $1/\lambda_{max} \Sigma_*$ and thus assume that $\lambda_{max} = 1$. Let $\lambda_{min}$ be the smallest non-zero eigenvalue of $\Sigma_*$. Then, $\lambda_{min} = \frac{1}{\kappa}$.

% Recall,  $\Sigma_* = U \Lambda U^{\top}$  and $\Pi_* = U U^{\top}$.
% Then, from the above, $\Sigma_* - \lambda_{min} \Pi_* \succeq 0$ and thus, using \eqref{fact:spectral-sos}, we have:
% \[
% \sststile{2}{v,\Pi} \Set{\lambda_{min} v^{\top}M \Pi_{*} Mv \leq v^{\top} M\Sigma_*Mv}\mper
% \]
% Using the \eqref{eq:sos-addition-multiplication-rule} repeatedly we thus obtain:
% \begin{equation}
% \label{eqn:lower_bound_on_quad}
% \sststile{k}{v} \Set{\lambda_{min}^{k/2} \Paren{v^{\top} M\Pi_{*}M v}^{k/2} \leq \Paren{v^{\top} M\Sigma_*Mv}^{k/2}}\mper
% \end{equation}
% Since $\lambda_{max} =1$ and $M^2 = M$, we have:
% \[
% \cA_{w,\Pi} \sststile{4}{v,\Pi} \Set{v^{\top} M \Sigma_* M v \leq \Norm{Mv}_2^2 =v^{\top}Mv = v^{\top} (\II-\Pi)v = \Norm{v}_2^2 - \Norm{\Pi v}_2^2\leq \Norm{v}_2^2}
% \]
% Using the \eqref{eq:sos-addition-multiplication-rule} repeatedly again, we  obtain:
% \begin{equation}
% \label{eqn:upper_bound_on_quad}
% \cA_{w,\Pi} \sststile{4}{v,\Pi} \Set{\Paren{v^{\top} M \Sigma_* M v}^{k/2} \leq \Norm{v}_2^k}
% \end{equation}
% Using \eqref{eqn:lower_bound_on_quad} and \eqref{eqn:upper_bound_on_quad}   with \eqref{eq:post-0-expression_3}, we thus have:
% \begin{equation}
% \label{eqn:quadatic_form_inequality}
% \cA_{w,\Pi} \sststile{2k}{v,w} \Set{w(\cI)^t \Paren{v^{\top} M\Pi_*M v}^{k/2} \leq \frac{1}{\lambda_{min}^{k/2}} w(\cI)^t \Paren{v^{\top} M\Sigma_*M v}^{k/2} \leq \frac{1}{\lambda_{min}^{k/2}} \delta^t \Norm{v}_2^{k}}\mper
% \end{equation}



Using \eqref{eq:sos-addition-multiplication-rule} and combining with \eqref{eq:bound_useful}, we thus obtain:
\[
\cA_{w,\Pi} \sststile{2k + t}{\Pi,w} \Set{ w(\cI)^t \Norm{\Pi-\Pi_*}_F^k = w(\cI)^t 2^{k/2} \Tr(M\Pi_*M)^{k/2} \leq (2r/\lambda_{min})^{k/2}\delta^t}\mper
\]
Noting that $\lambda_{min} = 1/\kappa$ completes the proof.
\end{proof}

\subsection{High-Entropy Pseudo-distributions: Proof of Lemma ~\ref{lem:high-entropy-pseudo-distributions}}
%\FIXME{this proof is too simple so we should just include it as an auxiliary lemma after all.}
% Thus far, we were able to upper bound $\|\Sig - \Sigma_*\|^2_F$ proportional to $\frac{1}{\sum_{i \in \cI} w_i}$. Apriori, the intersection of the indicator vector $w$ with the inliers may be $0$. Here we show that the intersection is in fact non-trivial.
% % The proof of this lemma follows from the following result proven in ~\cite{KKK19}.

\begin{fact}[Similar to the proof of Lemma 4.3 in ~\cite{DBLP:journals/corr/abs-1905-05679}]
Let $\tmu$ be a pseudo-distribution of degree at least $2$ on $w_1, w_2, \ldots, w_n$ that satisfies $\{w_i^2 = w_i \forall i\} \cup \{\sum_{i = 1}^n w_i = \alpha n\}$ and minimizes $\Norm{\sum_{i = 1}^n\pE[w_i]}^2_2$. Then, $\frac{1}{|\cI|}\sum_{i \in \cI} \pE[w_i] \geq \alpha$. \label{fact:KKK-high-entropy}
\end{fact}


\begin{proof}[Proof of Lemma \ref{lem:high-entropy-pseudo-distributions}]
From Fact~\ref{fact:KKK-high-entropy}, we have that $\frac{1}{|\cI|}\sum_{i \in \cI} \pE[w_i] \geq \alpha$.
Applying Hölder's inequality for pseudo-distributions with $f = 1$ and $g = \frac{1}{|\cI|} \sum_{i \in \cI} w_i$ gives:
\[
\frac{1}{|\cI|^t} \pE \Paren{\sum_{i \in \cI} w_i}^t \geq  \frac{1}{|\cI|^t}  \Paren{\sum_{i \in \cI}  \pE w_i}^t \geq \alpha^t\mper
\]
\end{proof}


\subsection{Rounding Pseudo-distributions to a Large List: Proof of Lemma ~\ref{lem:large-list-rounding}}


The key step in our proof is the following lemma:
\begin{lemma} \label{lem:step-1-large-rounding}
Given $t \in \N$, and an instance of $\sub_{\cD}(\alpha, \Sigma_*)$ such that $\cI$ is $k$-certifiably $(C, \delta)$-anti-concentrated, let $\tmu$ be a degree-$(2k+t)$ pseudo-distribution satisfying $\cA_{w,\Pi}$ and minimizing $\norm{\pE_{\tmu}{[w]}}_2$. Then,
\[
 \frac{ 1 }{\pE_{\tilde{\mu}} \left[\Paren{\sum_{i \in \cI} w_i}^t\right]} \sum_{S \subseteq \cI, |S|\leq t} {\cI \choose S} \pE_{\tilde{\mu}} \left[w_S \Norm{\Pi-\Pi_*}_F^k\right] \leq   \Paren{\frac{8\delta}{\alpha}}^t (2r \kappa)^{k/2}\mper
\]
where ${\cI \choose S}$ is the coefficient of the monomial indexed by $S$.
\end{lemma}

\begin{proof}
From Lemma~\ref{lem:main-sosized-fact}, we have for every $t,\ell \in \N$,
\begin{equation*}
\cA_{w,\Pi} \sststile{t+k}{w,\Pi} \left\{ \frac{ 1 }{|\I|^{t}} \Paren{\sum_{i \in \cI} w_i}^t  \Norm{\Pi-\Pi_*}_F^k \leq r(2r \kappa )^{k/2} \delta^t \right\} \mper
\end{equation*}
%\FIXME{add degree dependence on $\delta$}
Since $\tmu$ satisfies $\cA_{w,\Pi}$ and has degree at least $t+k$, taking pseudo-expectation yields:
\[
\pE_{\tmu} \left[ \frac{ 1 }{|\I|^{t}} \Paren{\sum_{i \in \cI} w_i}^t  \Norm{\Pi-\Pi_*}_F^k \right] \leq r (2r \kappa )^{k/2} \delta^t \mper
\]
Since $\tmu$ satisfies $\cA_{w,\Pi}$ and minimizes $\Norm{\pE_{\tilde{\mu}} w}_2$, Lemma~\ref{lem:high-entropy-pseudo-distributions} yields: $\frac{1}{|\cI|^t} \pE_{\tilde{\mu}} \left[ \Paren{\sum_{i \in \cI} w_i}^t \right] \geq \alpha^t$.
Multiplying both sides by $\frac{|\cI|^t}{\pE_{\tilde{\mu}} \left[\Paren{\sum_{i \in \cI} w_i}^t\right]}\leq \frac{1}{\alpha^t}$, we obtain:


\begin{equation}\label{eq:normalized-bound}
 \frac{ 1 }{\pE_{\tilde{\mu}} \left[\Paren{\sum_{i \in \cI} w_i}^t\right]} \pE_{\tmu}\left[\Paren{\sum_{i \in \cI} w_i}^t  \Norm{\Pi-\Pi_*}_F^k\right] \leq   \Paren{\frac{8\delta}{\alpha}}^t r (2r \kappa)^{k/2}\mper
\end{equation}

For any monomial $w_S$, let $w_{S'}$ be its multilinearization. Then, observe that:
\[
\Set{w_i^2=w_i \mid \forall i} \sststile{t}{w} \Set{ w_S = w_{S'}}\mper
\]
Therefore, we have
\begin{equation}
\label{eqn:expanding_to_monomial}
\cA_{w,\Pi} \sststile{t}{w} \Set{ \Paren{\sum_{i \in \cI} w_i}^t \Norm{\Pi-\Pi_*}_F^k = \sum_{S \subseteq \cI, |S| \leq t} {{\cI} \choose S} w_S \Norm{\Pi-\Pi_*}_F^k} \mper
\end{equation}
Combining equations \ref{eq:normalized-bound} and \ref{eqn:expanding_to_monomial}, we have
\begin{equation}\label{eq:final-bound}
 \frac{ 1 }{\pE_{\tilde{\mu}} \left[\Paren{\sum_{i \in \cI} w_i}^t\right]} \sum_{S \subseteq \cI, |S|\leq t} {\cI \choose S} \pE_{\tilde{\mu}} \left[w_S \Norm{\Pi-\Pi_*}_F^k\right] \leq   \Paren{\frac{8\delta}{\alpha}}^t r (2r \kappa)^{k/2}\mper
\end{equation}
which concludes the proof.







\end{proof}

Next, we show that sampling a subset of size $t$ indicated by thee $w$'s proportional to the marginal pseudo-distribution on this set results in an empirical estimator that is close to $\Pi_*$ with constant probability.

\begin{lemma}
\label{lem:key_rounding_lemma}
Given $t \in \mathbb{N}$, let $\tmu$ be a pseudo-distribution of degree at least $t +2k$ satisfying $\cA_{w,\Pi}$ and minimizing $\norm{\pE_{\tmu}{[w]}}_2$. Let $S \subseteq \cI$, $|S| \leq t$ be chosen randomly with probability proportional to ${\cI \choose S} \pE_{\tmu}[w_S]$. Let $\tmu_S$ be the pseudo-distribution obtained by reweighting $\tmu$ by the SoS polynomial $w_S^2$. Then, with probability at least $9/10$ over the draw of $S$, $\Norm{\pE_{\tmu_S}\left[ \Pi\right]-\Pi_*}_{F}^k \leq 10r (2r \kappa )^{k/2} (8\delta)^t \alpha^{-t}$.
\end{lemma}

\begin{proof}
Rewriting the conclusion of Lemma~\ref{lem:step-1-large-rounding}, we have:
\begin{equation}\label{eq:expectation-disguised}
\frac{1}{\pE_{\tilde{\mu}}\left[\Paren{\sum_{i \in \cI} w_i}^{t}\right]} \sum_{S \subseteq \cI, |S| \leq t} {\cI \choose S} \pE_{\tilde{\mu}}[w_S] \frac{\pE_{\tilde{\mu}}\left[w_S \Norm{\Pi-\Pi_*}_F^k\right]}{\pE_{\tilde{\mu}}[w_S]} \leq\Paren{\frac{8\delta}{\alpha}}^t r (2r \kappa)^{k/2}\mper
\end{equation}
Further, $\sum_{S \subseteq \cI, |S|\leq t} {\cI \choose  S} \pE_{\tilde{\mu}}[w_S] = \pE_{\tilde{\mu}}\Paren{\sum_{i \in \cI} w_i}^t$. Thus, $\frac{{\cI \choose  S} \pE_{\tilde{\mu}}[w_S] }{\pE_{\tilde{\mu}}\Paren{\sum_{i \in \cI} w_i}^t}$ is a probability distribution, $\zeta$, over $S \subseteq \cI, |S|\leq t$. Thus, we can rewrite \eqref{eq:expectation-disguised} as simply:
\[
\E_{S \sim \zeta} \left[\frac{\pE_{\tilde{\mu}}[w_S \Norm{\Pi-\Pi_*}_F^k]}{\pE_{\tilde{\mu}}[w_S]} \right]\leq  \Paren{\frac{8\delta}{\alpha}}^t r (2r \kappa)^{k/2}\mper
\]
By Markov's inequality, a $S \sim \zeta$ satisfies $\frac{\pE_{\tilde{\mu}}[w_S \Norm{\Pi-\Pi_*}_F^k]}{\pE[w_S]} \leq  10r (2r \kappa )^{k/2} (8\delta)^t \alpha^{-t}$ with probability at least $9/10$.
Finally, observe that by Fact~\ref{fact:reweightings}, $\pE_{\tmu_S} \Norm{\Pi-\Pi_*}_F^k = \frac{\pE_{\tilde{\mu}}[w_S \Norm{\Pi-\Pi_*}_F^k]}{\pE_{\tilde{\mu}}[w_S]}$. Thus, with probability at least $9/10$ over the choice of $S \sim \zeta$, $\pE_{\tmu_S} \left[\Norm{\Pi-\Pi_*}_F^k\right] \leq  10r (2r \kappa )^{k/2} (8\delta)^t \alpha^{-t}$.
By Cauchy-Schwarz inequality applied with $f=1$ and $g = \|(\Pi-\Pi_*)\|^k_F$, we have: $\Norm{\pE_{\tilde{\mu}}[(\Pi-\Pi_*)]}_F^k \leq \pE_{\tilde{\mu}} \left[\Norm{\Pi-\Pi_*}_F^k\right]$. Thus, $\Norm{\pE_{\tmu_S}\left[\Pi\right]-\Pi_*}_F^k \leq 10r (2r \kappa )^{k/2} (8\delta)^t \alpha^{-t}$. This completes the proof.

% Finally, using Lemma~\ref{lem:spectral-norm-vs-trace-powers} for the matrix $\pE_{\tmu_S}\Pi-\Sigma_*)$ yields:
% \[
% \Norm{\pE_{\tmu_S}\Sig - \Sigma_*}_{op} \leq \Paren{\Tr(\pE_{\tmu_S}\Pi-\Sigma_*)^{2\ell}}^{1/2\ell} \leq 4\Paren{\frac{\delta}{\alpha}}^{t/2\ell} r^{1/2\ell}\mper
% \]
\end{proof}


\begin{proof}[Proof of Lemma ~\ref{lem:large-list-rounding}]
We note that since $\cD$ is $k$-certifiably $(c,\delta)$-anti-concentrated, sampling $n_0 = (kd\log(d))^{k}$ suffices for the uniform distribution over $\cI$ to be $k$-certifiably $(c,2\delta)$-anti-concentrated (this follows from Lemma \ref{lem:certifiable_anti_conc_sampling}). 
We then observe that by Lemma \ref{fact:KKK-high-entropy}, $\frac{\pE_{\tmu}\left[(\sum_{i\in \cI} w_i)^t\right] }{|\cI|^t} = \frac{\pE_{\tmu}\left[(\sum_{i\in \cI} w_i)^t\right]}{\pE_{\tmu}\left[(\sum_{i\in [n]} w_i)^t\right] } \geq \alpha^{t}$. Therefore, with probability at least $9\alpha^t/10$, $w_S \subset \cI$ and the conclusion of Lemma \ref{lem:key_rounding_lemma} holds. However, the resulting matrix $\tilde{\Pi} = \pE_{\tmu_S}[\Pi]$ need not be a Projection matrix.


From Lemma \ref{lem:key_rounding_lemma}, we can now conclude $\norm{\tilde{\Pi} - \Pi_*}^2_F \leq \left(10r (2r \kappa )^{k/2} (8\delta/\alpha)^t \right)^{2/k} \leq c r^{1+1/k} \kappa (\delta/\alpha)^{2t/k} $. Setting $t = \Omega\left( \frac{k\log(r\kappa/\eta')}{\log(\delta/\alpha)}\right)$ in Lemma \ref{lem:key_rounding_lemma} suffices to bound $\norm{\tilde{\Pi} - \Pi_*}^2_F \leq \eta'$.
It follows that with probability at least $9\alpha^t/10$, for all $i\in[d]$, 
\[
\lambda^2_i(\tilde{\Pi}) = \lambda^2_i(\Pi_*) \pm \left(10r (2r \kappa )^{k/2} (8\delta)^t \alpha^{-t}\right) = \lambda^2_i(\Pi_*) \pm \eta'
\]
Since $\Pi_*$ is an actual rank-$r$ Projection matrix, for $i\in[r]$, $\lambda^2_i(\tilde{\Pi}) \in [1-\eta', 1+\eta']$ and for $i \in [r+1, d]$, $\lambda^2_i(\tilde{\Pi}) \in [-\eta', \eta']$ . Recall, $\tilde{\Pi} = U \Lambda U^{\top}$ is the full Eigenvalue decomposition and therefore, $\| (\Lambda -\II)\|^2_2 \leq \eta'$. Further, since $\sum^r_{i=1} \lambda^2_i(\tilde{\Pi}) \geq (1-\eta')r$ and trace is exactly $r$, $\|U_{\setminus r} \Lambda_{\setminus r} U^{\top}_{\setminus r} \|^2_F = \sum^{n}_{i=r+1} \lambda^2_i(\tilde{\Pi}) \leq r \eta'$. 

Now recall, $\hat{\Pi} = U_{r} U^{\top}_r$ is the corresponding Projection matrix we obtain in Algorithm \ref{alg:rounding_large_list}, where $U_{r}$ are the eigenvectors corresponding to the top-$r$ eigenvalues of $\tilde{\Pi}$. %Observe, $\norm{\hat{\Pi} - \tilde{\Pi}}^2_F = \sum_{i \in [d]} \lambda^2_i(\hat{\Pi} - \tilde{\Pi}) \leq 2d \eta'$.  
Therefore,
\begin{equation}
\begin{split}
\norm{\hat{\Pi} - \Pi_*}^2_F & = \norm{\hat{\Pi} - \tilde{\Pi}+ \tilde{\Pi}   - \Pi_*}^2_F  \\
& \leq 2\left(\norm{ \tilde{\Pi}    - \Pi_*}^2_F + \norm{ U_r U_r^{\top} - U\Lambda U^{\top} }^2_F  \right) \\
& \leq 4\left( \eta' + \norm{ U_r(\Lambda_r -\II_r)U_r^{\top} }^2_F +  \|U_{\setminus r} \Lambda_{\setminus r} U^{\top}_{\setminus r} \|^2_F \right) \\
& \leq 4\left( \eta' + \|(\Lambda_r -\II_r)\|^2_2 \norm{ \hat{\Pi} }^2_F +  r \eta' \right) \leq 6 r \eta'
\end{split}
\end{equation}
Setting $\eta' = \eta/6r$, we get $t =\Delta \left( \frac{k\log(r\kappa/\eta)}{\log(\delta/\alpha)}\right)$, for a sufficiently large constant $\Delta$.
Repeating $O(1/\alpha^t)$ times, with probability $99/100$, the resulting list contains a Projection matrix $\hat{\Pi}$ such that $\|\hat{\Pi} - \Pi_*\|^2_F \leq \eta$. The claim follows by choosing $\delta = \alpha/2$. The running time is dominated by computing a $(t + 2k)$-degree pseudo-distribution which requires $n^{O(k^2\log(r\kappa/\eta))}$ time.
\end{proof}



==> preamble/macros-custom.tex <==
% algorithm packages


%\usepackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{algpseudocode}

%\algnewcommand\algorithmicinput{\textbf{Input:}}
%\algnewcommand\INPUT{\item[\algorithmicinput]}
%\algnewcommand\algorithmicoutput{\textbf{Output:}}
%\algnewcommand\OUTPUT{\item[\algorithmicoutput]}

% paper-specific packages
\usepackage{relsize}
\usepackage[font=footnotesize]{caption}
\usepackage{appendix}


% abbreviations and paper-specific macros

% math
\newcommand{\D}{\mathcal{D}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\on}{\{-1,1\}}
\newcommand{\sphere}{\bbS^{n-1}}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\lamax}{\lambda_{\mathrm{max}}}
\newcommand{\Sn}{\mathbb{S}^{n-1}}
\DeclareMathOperator{\Id}{\mathrm{Id}}
\DeclareMathOperator{\F}{\mathbb{F}}
\DeclareMathOperator{\codim}{codim}


% not math
\DeclareUrlCommand\email{}
\newcommand{\whp}{\text{w.h.p.}}
\newcommand{\wovp}{\text{w.ov.p.}\xspace}
\newcommand{\YES}{\textsc{yes}\xspace}
\newcommand{\NO}{\textsc{no}\xspace}

\newcommand{\wovple}{\hspace{-3mm}\stackrel{\text{\wovp}}{\le}}
\newcommand{\wovpeq}{\hspace{-3mm}\stackrel{\text{\wovp}}{=}}
\newcommand{\wovpge}{\hspace{-3mm}\stackrel{\text{\wovp}}{\ge}}
\newcommand{\aasle}{\hspace{-1.5mm}\stackrel{\text{a.a.s.}}\le}

\newcommand{\Pisymm}{\Pi_{\mathrm{symm}}}
\newcommand{\Pisym}{\Pi_{\mathrm{sym}}}

%added by TM
\newcommand{\inner}[1]{\langle #1 \rangle}
\newcommand{\sosle}{\preceq}
\newcommand{\sosge}{\succeq}

\DeclareMathOperator{\tE}{\tilde{\mathbb E}}
\DeclareMathOperator{\tO}{\tilde{O}}
\newcommand{\ta}{\tilde{a}}
\newcommand{\tA}{\tilde{A}}


\DeclareMathOperator*{\pE}{\tilde{\mathbb E}}

\newcommand{\bT}{\mathbf{T}}
\newcommand{\ot}{\otimes}
\newcommand{\tr}{\textup{tr}}
\newcommand{\diag}{\textup{diag}}

\let\pref=\prettyref

% transpose
% http://tex.stackexchange.com/questions/204892/visually-appealing-subscripts-with-intercal
% http://tex.stackexchange.com/questions/30619/what-is-the-best-symbol-for-vector-matrix-transpose
\newcommand*{\transpose}[1]{{#1}{}^{\mkern-4mu\intercal}}
\newcommand*{\vardyad}[1]{#1^{\vphantom{\intercal}}#1^{\intercal}}
\newcommand*{\dyad}[1]{#1#1{}^{\mkern-4mu\intercal}}

% \let\Id\undefined
% \newcommand*{\Id}{I}

% span of subspace -- temporary

\newcommand{\sspan}{\textup{span}}
\newcommand{\1}{\bm{1}}

\newcommand{\Cov}{\mathop{\mathrm{Cov}}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../planted"
%%% End:


==> preamble/macros.tex <==
% {{{ etex }}}

\usepackage{etex}

% {{{ nag }}}

\usepackage[l2tabu, orthodox]{nag}

% {{{ common }}}

\usepackage{xspace,enumerate}

\usepackage[dvipsnames]{xcolor}

\usepackage[T1]{fontenc}
\usepackage[full]{textcomp}

% {{{ babelamerican }}}
\usepackage[american]{babel}

% {{{ mathtools }}}

\usepackage{mathtools}


% {{{ boldmath }}}

% fix for "too many math alphabets" problem
\newcommand\hmmax{0} % default 3
% \usepackage{bm}

% \usepackage{stmaryrd}


% {{{ amsthm }}}
\usepackage{amsthm}

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}

\newtheorem{subclaim}{Claim}[theorem]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newtheorem*{fact*}{Fact}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem*{hypothesis*}{Hypothesis}
\newtheorem{conjecture}[theorem]{Conjecture}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{example}[theorem]{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{protocol}[theorem]{Protocol}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem*{claim*}{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{observation}[theorem]{Observation}
\newtheorem*{observation*}{Observation}



% {{{ geometry-nice }}}


\ifnum\writemode=1
\usepackage[
letterpaper,
top=1.2in,
bottom=1.2in,
left=1in,
right=1in]{geometry}

\pagestyle{empty}
\fi

\ifnum\writemode=0
\usepackage[
letterpaper,
top=0.7in,
bottom=0.9in,
left=1in,
right=1in]{geometry}
\fi

% {{{ fonts }}}

\usepackage{newpxtext} % T1, lining figures in math, osf in text
\usepackage{textcomp} % required for special glyphs
\usepackage[varg,bigdelims]{newpxmath}
\usepackage[scr=rsfso]{mathalfa}% \mathscr is fancier than \mathcal
\usepackage{bm} % load after all math to give access to bold math
% \useosf %no longer needed
\linespread{1.1}% Give Palatino more leading (space between lines)
\let\mathbb\varmathbb

% {{{ showkeys }}}

\ifnum\showkeys=1
\usepackage[color]{showkeys}
\fi

% {{{ hyperref-option2 }}}

\ifnum\showcolorlinks=1
\usepackage[
pagebackref,
% letterpaper=true,
colorlinks=true,
urlcolor=blue,
linkcolor=blue,
citecolor=OliveGreen,
]{hyperref}
\fi

\ifnum\showcolorlinks=0
\usepackage[
pagebackref,
% letterpaper=true,
colorlinks=false,
pdfborder={0 0 0}
]{hyperref}
\fi


\usepackage[capitalise,nameinlink]{cleveref}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{definition}{Definition}{Definitions}

% {{{ prettyref }}}

% \usepackage{prettyref}

% % From manual:
% % \newrefformat{eq}{\textup{(\ref{#1})}}
% % \newrefformat{lem}{Lemma~\ref{#1}}
% % \newrefformat{thm}{Theorem~\ref{#1}}
% % \newrefformat{cha}{Chapter~\ref{#1}}
% % \newrefformat{sec}{Section~\ref{#1}}
% % \newrefformat{tab}{Table~\ref{#1} on page~\pageref{#1}}
% % \newrefformat{fig}{Figure~\ref{#1} on page~\pageref{#1}}

% \newcommand{\savehyperref}[2]{\texorpdfstring{\hyperref[#1]{#2}}{#2}}

% \newrefformat{eq}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
% \newrefformat{eqn}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
% \newrefformat{lem}{\savehyperref{#1}{Lemma~\ref*{#1}}}
% \newrefformat{def}{\savehyperref{#1}{Definition~\ref*{#1}}}
% \newrefformat{thm}{\savehyperref{#1}{Theorem~\ref*{#1}}}
% \newrefformat{cor}{\savehyperref{#1}{Corollary~\ref*{#1}}}
% \newrefformat{cha}{\savehyperref{#1}{Chapter~\ref*{#1}}}
% \newrefformat{sec}{\savehyperref{#1}{Section~\ref*{#1}}}
% \newrefformat{app}{\savehyperref{#1}{Appendix~\ref*{#1}}}
% \newrefformat{tab}{\savehyperref{#1}{Table~\ref*{#1}}}
% \newrefformat{fig}{\savehyperref{#1}{Figure~\ref*{#1}}}
% \newrefformat{hyp}{\savehyperref{#1}{Hypothesis~\ref*{#1}}}
% \newrefformat{alg}{\savehyperref{#1}{Algorithm~\ref*{#1}}}
% \newrefformat{rem}{\savehyperref{#1}{Remark~\ref*{#1}}}
% \newrefformat{item}{\savehyperref{#1}{Item~\ref*{#1}}}
% \newrefformat{step}{\savehyperref{#1}{step~\ref*{#1}}}
% \newrefformat{conj}{\savehyperref{#1}{Conjecture~\ref*{#1}}}
% \newrefformat{fact}{\savehyperref{#1}{Fact~\ref*{#1}}}
% \newrefformat{prop}{\savehyperref{#1}{Proposition~\ref*{#1}}}
% \newrefformat{prob}{\savehyperref{#1}{Problem~\ref*{#1}}}
% \newrefformat{claim}{\savehyperref{#1}{Claim~\ref*{#1}}}
% \newrefformat{relax}{\savehyperref{#1}{Relaxation~\ref*{#1}}}
% \newrefformat{red}{\savehyperref{#1}{Reduction~\ref*{#1}}}
% \newrefformat{part}{\savehyperref{#1}{Part~\ref*{#1}}}



% {{{ sref }}}

% short section reference
\newcommand{\Sref}[1]{\hyperref[#1]{\S\ref*{#1}}}

% {{{ nicefrac }}}
% commands for fractions
\usepackage{nicefrac}
% poor man's fraction
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\varflatfrac}[2]{#1\textfractionsolidus#2}

\let\nfrac=\nicefrac
\let\ffrac=\flatfrac
% similar commands: tfrac,dfrac

\newcommand{\half}{\nicefrac12}
\newcommand{\onequarter}{\nicefrac14}
\newcommand{\threequarter}{\nicefrac34}

% {{{ microtype-option }}}

\ifnum\usemicrotype=1
\usepackage{microtype}
\fi

% {{{ authornotes }}}
\ifnum\showauthornotes=1
\newcommand{\Authornote}[2]{{\sffamily\small\color{red}{[#1: #2]}}}
\newcommand{\Authornotecolored}[3]{{\sffamily\small\color{#1}{[#2: #3]}}}
\newcommand{\Authorcomment}[2]{{\sffamily\small\color{gray}{[#1: #2]}}}
\newcommand{\Authorstartcomment}[1]{\sffamily\small\color{gray}[#1: }
\newcommand{\Authorendcomment}{]\rmfamily\normalsize\color{black}}
\newcommand{\Authorfnote}[2]{\footnote{\color{red}{#1: #2}}}
\newcommand{\Authorfixme}[1]{\Authornote{#1}{\textbf{??}}}
\newcommand{\Authormarginmark}[1]{\marginpar{\textcolor{red}{\fbox{\Large #1:!}}}}
\else
\newcommand{\Authornote}[2]{}
\newcommand{\Authornotecolored}[3]{}
\newcommand{\Authorcomment}[2]{}
\newcommand{\Authorstartcomment}[1]{}
\newcommand{\Authorendcomment}{}
\newcommand{\Authorfnote}[2]{}
\newcommand{\Authorfixme}[1]{}
\newcommand{\Authormarginmark}[1]{}
\fi

\newcommand{\Dnote}{\Authornote{D}}
%\newcommand{\Tnote}{\Authornotecolored{blue}{T}}
\newcommand{\TMnote}{\Authornotecolored{blue}{T}}
\newcommand{\Inote}{\Authornotecolored{ForestGreen}{I}}
\newcommand{\inote}{\Inote}
\newcommand{\Gnote}{\Authornote{G}}
\newcommand{\Jcomment}{\Authorcomment{J}}
\newcommand{\Dcomment}{\Authorcomment{D}}
\newcommand{\Dstartcomment}{\Authorstartcomment{D}}
\newcommand{\Dendcomment}{\Authorendcomment}
\newcommand{\Dfixme}{\Authorfixme{D}}
\newcommand{\Dmarginmark}{\Authormarginmark{D}}
\newcommand{\Dfnote}{\Authorfnote{D}}

\newcommand{\Pnote}{\Authornote{P}}
\newcommand{\Pfnote}{\Authorfnote{P}}

\newcommand{\PRnote}{\Authornote{PR}}
\newcommand{\PRfnote}{\Authorfnote{PR}}

\newcommand{\PTnote}{\Authornote{PT}}
\newcommand{\PTfnote}{\Authorfnote{PT}}

\newcommand{\PGnote}{\Authornote{PG}}
\newcommand{\PGfnote}{\Authorfnote{PG}}

\newcommand{\Bnote}{\Authornote{B}}
\newcommand{\Bfnote}{\Authorfnote{B}}

\definecolor{forestgreen(traditional)}{rgb}{0.0, 0.27, 0.13}
\newcommand{\Jnote}{\Authornotecolored{forestgreen(traditional)}{J}}
\newcommand{\Jfnote}{\Authorfnote{J}}


\newcommand{\Mnote}{\Authornote{M}}
\newcommand{\Mfnote}{\Authorfnote{M}}

\newcommand{\Rnote}{\Authornote{M}}
\newcommand{\Rfnote}{\Authorfnote{M}}

\newcommand{\Nnote}{\Authornote{N}}
\newcommand{\Nfnote}{\Authorfnote{N}}

\newcommand{\Snote}{\Authornote{S}}
\newcommand{\Sfnote}{\Authorfnote{S}}


% {{{ fixme }}}

% place red exclamation mark in margin
%\newcommand{\redmarginmarker}{\marginpar{\textcolor{red}{\fbox{\Large !}}}}
\newcommand{\redmarginmarker}{}

% short indicator for places that need fixing
\newcommand{\FIXME}{\textbf{\textcolor{red}{??}}\redmarginmarker}

\ifnum\showfixme=0
\renewcommand{\FIXME}{}
\fi


% {{{ boxedminipage }}}
\usepackage{boxedminipage}

\newenvironment{mybox}
{\center \noindent\begin{boxedminipage}{1.0\linewidth}}
{\end{boxedminipage}
\noindent
}


% {{{ parentheses }}}
% various bracket-like commands
% round parentheses
\newcommand{\paren}[1]{(#1)}
\newcommand{\Paren}[1]{\left(#1\right)}
\newcommand{\bigparen}[1]{\big(#1\big)}
\newcommand{\Bigparen}[1]{\Big(#1\Big)}
% square brackets
\newcommand{\brac}[1]{[#1]}
\newcommand{\Brac}[1]{\left[#1\right]}
\newcommand{\bigbrac}[1]{\big[#1\big]}
\newcommand{\Bigbrac}[1]{\Big[#1\Big]}
\newcommand{\Biggbrac}[1]{\Bigg[#1\Bigg]}
% absolute value
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigabs}[1]{\big\lvert#1\big\rvert}
\newcommand{\Bigabs}[1]{\Big\lvert#1\Big\rvert}
% cardinality
\newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\Card}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigcard}[1]{\big\lvert#1\big\rvert}
\newcommand{\Bigcard}[1]{\Big\lvert#1\Big\rvert}
% set
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\bigset}[1]{\big\{#1\big\}}
\newcommand{\Bigset}[1]{\Big\{#1\Big\}}
% norm
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bignorm}[1]{\big\lVert#1\big\rVert}
\newcommand{\Bignorm}[1]{\Big\lVert#1\Big\rVert}
\newcommand{\Biggnorm}[1]{\Bigg\lVert#1\Bigg\rVert}
% 2-norm
\newcommand{\normt}[1]{\norm{#1}_2}
\newcommand{\Normt}[1]{\Norm{#1}_2}
\newcommand{\bignormt}[1]{\bignorm{#1}_2}
\newcommand{\Bignormt}[1]{\Bignorm{#1}_2}
% 2-norm squared
\newcommand{\snormt}[1]{\norm{#1}^2_2}
\newcommand{\Snormt}[1]{\Norm{#1}^2_2}
\newcommand{\bigsnormt}[1]{\bignorm{#1}^2_2}
\newcommand{\Bigsnormt}[1]{\Bignorm{#1}^2_2}
% norm squared
\newcommand{\snorm}[1]{\norm{#1}^2}
\newcommand{\Snorm}[1]{\Norm{#1}^2}
\newcommand{\bigsnorm}[1]{\bignorm{#1}^2}
\newcommand{\Bigsnorm}[1]{\Bignorm{#1}^2}
% 1-norm
\newcommand{\normo}[1]{\norm{#1}_1}
\newcommand{\Normo}[1]{\Norm{#1}_1}
\newcommand{\bignormo}[1]{\bignorm{#1}_1}
\newcommand{\Bignormo}[1]{\Bignorm{#1}_1}
% infty-norm
\newcommand{\normi}[1]{\norm{#1}_\infty}
\newcommand{\Normi}[1]{\Norm{#1}_\infty}
\newcommand{\bignormi}[1]{\bignorm{#1}_\infty}
\newcommand{\Bignormi}[1]{\Bignorm{#1}_\infty}
% inner product
\newcommand{\iprod}[1]{\langle#1\rangle}
\newcommand{\Iprod}[1]{\left\langle#1\right\rangle}
\newcommand{\bigiprod}[1]{\big\langle#1\big\rangle}
\newcommand{\Bigiprod}[1]{\Big\langle#1\Big\rangle}


% {{{ probability }}}
% expectation, probability, variance
\newcommand{\Esymb}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathbb{V}}

\DeclareMathOperator*{\E}{\Esymb}
\DeclareMathOperator*{\Var}{\Vsymb}
\DeclareMathOperator*{\ProbOp}{\Psymb}

\renewcommand{\Pr}{\ProbOp}

% TODO: make case distinction if optional argument is not set
\newcommand{\prob}[1]{\Pr\set{#1}}
\newcommand{\Prob}[2][]{\Pr_{{#1}}\Set{#2}}

\newcommand{\ex}[1]{\E\brac{#1}}
\newcommand{\Ex}[2][]{\E_{{#1}}\Brac{#2}}
\newcommand{\varex}[1]{\E\paren{#1}}
\newcommand{\varEx}[1]{\E\Paren{#1}}

%\newcommand{\given}{\;\middle\vert\;}
\newcommand{\given}{\mathrel{}\middle\vert\mathrel{}}
%\newcommand{\given}{\mathrel{}\middle|\mathrel{}}

% {{{ mathfonts }}}

% \usepackage{dsfont}
% \usepackage{yfonts}
% \usepackage{mathrsfs}


% {{{ miscmacros }}}

% middle delimiter in the definition of a set
\newcommand{\suchthat}{\;\middle\vert\;}

% tensor product
\newcommand{\tensor}{\otimes}

% add explanations to math displays
\newcommand{\where}{\text{where}}
\newcommand{\textparen}[1]{\text{(#1)}}
\newcommand{\using}[1]{\textparen{using #1}}
\newcommand{\smallusing}[1]{\text{(\small using #1)}}
\ifx\because\undefined
\newcommand{\because}[1]{\textparen{because #1}}
\else
\renewcommand{\because}[1]{\textparen{because #1}}
\fi
\newcommand{\by}[1]{\textparen{by #1}}


% spectral order (Loewner order)
\newcommand{\sge}{\succeq}
\newcommand{\sle}{\preceq}

% smallest and largest eigenvalue
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\lmax}{\lambda_{\max}}

\newcommand{\signs}{\set{1,-1}}
\newcommand{\varsigns}{\set{\pm 1}}
\newcommand{\maximize}{\mathop{\textrm{maximize}}}
\newcommand{\minimize}{\mathop{\textrm{minimize}}}
\newcommand{\subjectto}{\mathop{\textrm{subject to}}}

\renewcommand{\ij}{{ij}}

% symmetric difference
\newcommand{\symdiff}{\Delta}
\newcommand{\varsymdiff}{\bigtriangleup}

% set of bits
\newcommand{\bits}{\{0,1\}}
\newcommand{\sbits}{\{\pm1\}}

% no stupid bullets for itemize environmentx
% \renewcommand{\labelitemi}{--}

% control white space of list and display environments
\newcommand{\listoptions}{\labelsep0mm\topsep-0mm\itemindent-6mm\itemsep0mm}
\newcommand{\displayoptions}[1]{\abovedisplayshortskip#1mm\belowdisplayshortskip#1mm\abovedisplayskip#1mm\belowdisplayskip#1mm}

% short for emptyset
%\newcommand{\eset}{\emptyset}
% moved to mathabbreviations

% short for epsilon
%\newcommand{\e}{\epsilon}
% moved to mathabbreviations

% super index with parentheses
\newcommand{\super}[2]{#1^{\paren{#2}}}
\newcommand{\varsuper}[2]{#1^{\scriptscriptstyle\paren{#2}}}

% tensor power notation
\newcommand{\tensorpower}[2]{#1^{\tensor #2}}


% multiplicative inverse
\newcommand{\inv}[1]{{#1^{-1}}}

% dual element
\newcommand{\dual}[1]{{#1^*}}

% subset
%\newcommand{\sse}{\subseteq}
% moved to mathabbreviations

% vertical space in math formula
\newcommand{\vbig}{\vphantom{\bigoplus}}

% setminus
\newcommand{\sm}{\setminus}

% define something by an equation (display)
\newcommand{\defeq}{\stackrel{\mathrm{def}}=}


% define something by an equation (inline)
\newcommand{\seteq}{\mathrel{\mathop:}=}



% declare function f by $f \from X \to Y$
\newcommand{\from}{\colon}

% big middle separator (for conditioning probability spaces)
\newcommand{\bigmid}{~\big|~}
\newcommand{\Bigmid}{~\Big|~}
\newcommand{\Mid}{\;\middle\vert\;}

% better vector definition and some variations
%\renewcommand{\vec}[1]{{\bm{#1}}}
\newcommand{\bvec}[1]{\bar{\vec{#1}}}
\newcommand{\pvec}[1]{\vec{#1}'}
\newcommand{\tvec}[1]{{\tilde{\vec{#1}}}}

% punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

% inner product for matrices
\newcommand\bdot\bullet

% transpose
\newcommand{\trsp}[1]{{#1}^\dagger}

% indicator function / vector
\ifx\mathds\undefined % use double stroke fonts if available
\DeclareMathOperator{\Ind}{\mathbb{I}}
\else
\DeclareMathOperator{\Ind}{\mathds 1}}
\fi

% place a qed symbol inside display formula
%\qedhere

% {{{ superscripts }}}

\renewcommand{\th}{\textsuperscript{th}\xspace}
\newcommand{\st}{\textsuperscript{st}\xspace}
\newcommand{\nd}{\textsuperscript{nd}\xspace}
\newcommand{\rd}{\textsuperscript{rd}\xspace}


% {{{ mathoperators }}}
\DeclareMathOperator{\Inf}{Inf}
\DeclareMathOperator{\Tr}{Tr}
%\newcommand{\Tr}{\mathrm{Tr}}
\DeclareMathOperator{\SDP}{SDP}
\DeclareMathOperator{\sdp}{sdp}
\DeclareMathOperator{\val}{val}
\DeclareMathOperator{\LP}{LP}
\DeclareMathOperator{\OPT}{OPT}
\DeclareMathOperator{\opt}{opt}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\qpoly}{qpoly}
\DeclareMathOperator{\qpolylog}{qpolylog}
\DeclareMathOperator{\qqpoly}{qqpoly}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\Conv}{Conv}

\DeclareMathOperator{\rank}{rank}

% operators with limits
\DeclareMathOperator*{\median}{median}
\DeclareMathOperator*{\Median}{Median}

% smaller summation/product symbols
\DeclareMathOperator*{\varsum}{{\textstyle \sum}}
\DeclareMathOperator{\tsum}{{\textstyle \sum}}

\let\varprod\undefined

\DeclareMathOperator*{\varprod}{{\textstyle \prod}}
\DeclareMathOperator{\tprod}{{\textstyle \prod}}




% {{{ differentials }}}

\newcommand{\diffmacro}[1]{\,\mathrm{d}#1}

\newcommand{\dmu}{\diffmacro{\mu}}
\newcommand{\dgamma}{\diffmacro{\gamma}}
\newcommand{\dlambda}{\diffmacro{\lambda}}
\newcommand{\dx}{\diffmacro{x}}
\newcommand{\dt}{\diffmacro{t}}



% {{{ textabbreviations }}}

% some abbreviations
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\Eg}{E.g.,\xspace}
\newcommand{\phd}{Ph.\,D.\xspace}
\newcommand{\msc}{M.\,S.\xspace}
\newcommand{\bsc}{B.\,S.\xspace}

\newcommand{\etal}{et al.\xspace}

\newcommand{\iid}{i.i.d.\xspace}

% {{{ foreignwords }}}

\newcommand\naive{na\"{\i}ve\xspace}
\newcommand\Naive{Na\"{\i}ve\xspace}
\newcommand\naively{na\"{\i}vely\xspace}
\newcommand\Naively{Na\"{\i}vely\xspace}




% {{{ names }}}
% Hungarian/Polish/East European names
\newcommand{\Erdos}{Erd\H{o}s\xspace}
\newcommand{\Renyi}{R\'enyi\xspace}
\newcommand{\Lovasz}{Lov\'asz\xspace}
\newcommand{\Juhasz}{Juh\'asz\xspace}
\newcommand{\Bollobas}{Bollob\'as\xspace}
\newcommand{\Furedi}{F\"uredi\xspace}
\newcommand{\Komlos}{Koml\'os\xspace}
\newcommand{\Luczak}{\L uczak\xspace}
\newcommand{\Kucera}{Ku\v{c}era\xspace}
\newcommand{\Szemeredi}{Szemer\'edi\xspace}
\newcommand{\Hastad}{H{\aa}stad\xspace}
\newcommand{\Hoelder}{H\"{o}lder\xspace}
\newcommand{\Holder}{\Hoelder}
\newcommand{\Brandao}{Brand\~ao\xspace}


% {{{ numbersets }}}
% number sets
\newcommand{\Z}{\mathbb Z}
\newcommand{\N}{\mathbb N}
\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\Rnn}{\R_+}
\newcommand{\varR}{\Re}
\newcommand{\varRnn}{\varR_+}
\newcommand{\varvarRnn}{\R_{\ge 0}}


% {{{ problems }}}

% macros to denote computational problems

% use texorpdfstring to avoid problems with hyperref (can use problem
% macros also in headings
\newcommand{\problemmacro}[1]{\texorpdfstring{\textup{\textsc{#1}}}{#1}\xspace}

\newcommand{\pnum}[1]{{\footnotesize #1}}

% list of problems
\newcommand{\uniquegames}{\problemmacro{unique games}}
\newcommand{\maxcut}{\problemmacro{max cut}}
\newcommand{\multicut}{\problemmacro{multi cut}}
\newcommand{\vertexcover}{\problemmacro{vertex cover}}
\newcommand{\balancedseparator}{\problemmacro{balanced separator}}
\newcommand{\maxtwosat}{\problemmacro{max \pnum{3}-sat}}
\newcommand{\maxthreesat}{\problemmacro{max \pnum{3}-sat}}
\newcommand{\maxthreelin}{\problemmacro{max \pnum{3}-lin}}
\newcommand{\threesat}{\problemmacro{\pnum{3}-sat}}
\newcommand{\labelcover}{\problemmacro{label cover}}
\newcommand{\setcover}{\problemmacro{set cover}}
\newcommand{\maxksat}{\problemmacro{max $k$-sat}}
\newcommand{\mas}{\problemmacro{maximum acyclic subgraph}}
\newcommand{\kwaycut}{\problemmacro{$k$-way cut}}
\newcommand{\sparsestcut}{\problemmacro{sparsest cut}}
\newcommand{\betweenness}{\problemmacro{betweenness}}
\newcommand{\uniformsparsestcut}{\problemmacro{uniform sparsest cut}}
\newcommand{\grothendieckproblem}{\problemmacro{Grothendieck problem}}
\newcommand{\maxfoursat}{\problemmacro{max \pnum{4}-sat}}
\newcommand{\maxkcsp}{\problemmacro{max $k$-csp}}
\newcommand{\maxdicut}{\problemmacro{max dicut}}
\newcommand{\maxcutgain}{\problemmacro{max cut gain}}
\newcommand{\smallsetexpansion}{\problemmacro{small-set expansion}}
\newcommand{\minbisection}{\problemmacro{min bisection}}
\newcommand{\minimumlineararrangement}{\problemmacro{minimum linear arrangement}}
\newcommand{\maxtwolin}{\problemmacro{max \pnum{2}-lin}}
\newcommand{\gammamaxlin}{\problemmacro{$\Gamma$-max \pnum{2}-lin}}
\newcommand{\basicsdp}{\problemmacro{basic sdp}}
\newcommand{\dgames}{\problemmacro{$d$-to-1 games}}
\newcommand{\maxclique}{\problemmacro{max clique}}
\newcommand{\densestksubgraph}{\problemmacro{densest $k$-subgraph}}


% {{{ alphabet }}}

\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}
\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}
\newcommand{\cH}{\mathcal H}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}
\newcommand{\cL}{\mathcal L}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cR}{\mathcal R}
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}

\newcommand{\scrA}{\mathscr A}
\newcommand{\scrB}{\mathscr B}
\newcommand{\scrC}{\mathscr C}
\newcommand{\scrD}{\mathscr D}
\newcommand{\scrE}{\mathscr E}
\newcommand{\scrF}{\mathscr F}
\newcommand{\scrG}{\mathscr G}
\newcommand{\scrH}{\mathscr H}
\newcommand{\scrI}{\mathscr I}
\newcommand{\scrJ}{\mathscr J}
\newcommand{\scrK}{\mathscr K}
\newcommand{\scrL}{\mathscr L}
\newcommand{\scrM}{\mathscr M}
\newcommand{\scrN}{\mathscr N}
\newcommand{\scrO}{\mathscr O}
\newcommand{\scrP}{\mathscr P}
\newcommand{\scrQ}{\mathscr Q}
\newcommand{\scrR}{\mathscr R}
\newcommand{\scrS}{\mathscr S}
\newcommand{\scrT}{\mathscr T}
\newcommand{\scrU}{\mathscr U}
\newcommand{\scrV}{\mathscr V}
\newcommand{\scrW}{\mathscr W}
\newcommand{\scrX}{\mathscr X}
\newcommand{\scrY}{\mathscr Y}
\newcommand{\scrZ}{\mathscr Z}

\newcommand{\bbB}{\mathbb B}
\newcommand{\bbS}{\mathbb S}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbI}{\mathbb I}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbP}{\mathbb P}
\newcommand{\bbE}{\mathbb E}
\newcommand{\bbN}{\mathbb N}

\newcommand{\sfE}{\mathsf E}


% {{{ leqslant }}}
% slanted lower/greater equal signs
\renewcommand{\leq}{\leqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\ge}{\geqslant}


% {{{ draftbox }}}
\ifnum\showdraftbox=1
\newcommand{\draftbox}{\begin{center}
  \fbox{%
    \begin{minipage}{2in}%
      \begin{center}%
%        \begin{Large}%
          \Large\textsc{Working Draft}\\%
%        \end{Large}\\
        Please do not distribute%
      \end{center}%
    \end{minipage}%
  }%
\end{center}
\vspace{0.2cm}}
\else
\newcommand{\draftbox}{}
\fi


% {{{ varepsilon }}}

\let\epsilon=\varepsilon

% {{{ numberequationwithinsection }}}
\numberwithin{equation}{section}


% {{{ restate }}}
% set of macros to deal with restating theorem environments (or anything
% else with a label)

% stolen from Boaz's latex macros

\newcommand\MYcurrentlabel{xxx}

% \MYstore{A}{B} assigns variable A value B
\newcommand{\MYstore}[2]{%
  \global\expandafter \def \csname MYMEMORY #1 \endcsname{#2}%
}

% \MYload{A} outputs value stored for variable A
\newcommand{\MYload}[1]{%
  \csname MYMEMORY #1 \endcsname%
}

% new label command, stores current label in \MYcurrentlabel
\newcommand{\MYnewlabel}[1]{%
  \renewcommand\MYcurrentlabel{#1}%
  \MYoldlabel{#1}%
}

% new label command that doesn't do anything
\newcommand{\MYdummylabel}[1]{}

\newcommand{\torestate}[1]{%
  % overwrite label command
  \let\MYoldlabel\label%
  \let\label\MYnewlabel%
  #1%
  \MYstore{\MYcurrentlabel}{#1}%
  % restore old label command
  \let\label\MYoldlabel%
}

\newcommand{\restatetheorem}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{theorem*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{theorem*}
  \let\label\MYoldlabel
}

\newcommand{\restatelemma}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{lemma*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{lemma*}
  \let\label\MYoldlabel
}

\newcommand{\restateprop}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{proposition*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{proposition*}
  \let\label\MYoldlabel
}

\newcommand{\restatefact}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{fact*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{fact*}
  \let\label\MYoldlabel
}

\newcommand{\restate}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \MYload{#1}
  \let\label\MYoldlabel
}


% {{{ bibliography }}}

% add section for references to table of contents
\newcommand{\addreferencesection}{
  \phantomsection
  \addcontentsline{toc}{section}{References}
}


% {{{ mathabbreviations }}}

\newcommand{\la}{\leftarrow}
\newcommand{\sse}{\subseteq}
\newcommand{\ra}{\rightarrow}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\eset}{\emptyset}


% {{{ paragraphperiod }}}


\let\origparagraph\paragraph
\renewcommand{\paragraph}[1]{\origparagraph{#1.}}


% {{{ allowdisplaybreaks }}}
% allows page breaks in large display math formulas

\allowdisplaybreaks


% {{{ sloppy }}}
% avoid math spilling on margin

\sloppy

% {{{ complexityclasses }}}

\newcommand{\cclassmacro}[1]{\texorpdfstring{\textbf{#1}}{#1}\xspace}
\newcommand{\p}{\cclassmacro{P}}
\newcommand{\np}{\cclassmacro{NP}}
\newcommand{\subexp}{\cclassmacro{SUBEXP}}

% {{{ paralist }}}

\usepackage{paralist}

% {{{ comment }}}

\usepackage{comment}


%{{{Bra Ket Notation}}}
\usepackage{braket}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../planted"
%%% End:

